Efficient Frameworks for Generalized Low-Rank Matrix Bandit Problems

In the stochastic contextual low-rank matrix bandit problem, the expected reward of an action is given by the inner product between the action's feature matrix and some fixed, but initially unknown $d_1$ by $d_2$ matrix $\Theta^*$ with rank $r \ll \{d_1, d_2\}$, and an agent sequentially takes actions based on past experience to maximize the cumulative reward. In this paper, we study the generalized low-rank matrix bandit problem, which has been recently proposed in \cite{lu2021low} under the Generalized Linear Model (GLM) framework. To overcome the computational infeasibility and theoretical restrain of existing algorithms on this problem, we first propose the G-ESTT framework that modifies the idea from \cite{jun2019bilinear} by using Stein's method on the subspace estimation and then leverage the estimated subspaces via a regularization idea. Furthermore, we remarkably improve the efficiency of G-ESTT by using a novel exclusion idea on the estimated subspace instead, and propose the G-ESTS framework. We also show that G-ESTT can achieve the $\tilde{O}(\sqrt{(d_1+d_2)MrT})$ bound of regret while G-ESTS can achineve the $\tilde{O}(\sqrt{(d_1+d_2)^{3/2}Mr^{3/2}T})$ bound of regret under mild assumption up to logarithm terms, where $M$ is some problem dependent value. Under a reasonable assumption that $M = O((d_1+d_2)^2)$ in our problem setting, the regret of G-ESTT is consistent with the current best regret of $\tilde{O}((d_1+d_2)^{3/2} \sqrt{rT}/D_{rr})$~\citep{lu2021low} ($D_{rr}$ will be defined later). For completeness, we conduct experiments to illustrate that our proposed algorithms, especially G-ESTS, are also computationally tractable and consistently outperform other state-of-the-art (generalized) linear matrix bandit methods based on a suite of simulations.

==> app_assu.tex <==
\section{Details of Assumption \ref{assu_sampling}-\ref{assu_link}}\label{app:assu}
Here are some comments or remarks about Assumptions \ref{assu_sampling}-\ref{assu_link}, which further imply that our assumptions are mild and standard.
\begin{enumerate}
\item The Assumption \ref{assu_sampling} is very mild since based on the properties of sub-Gaussian distribution and Orcliz-2 norm we can always choose appropriate values for $\lambda_1$ and $\lambda_2$ in most cases~\citep{wainwright2019high}. In \ref{sec:pre} we denote $\lambda_2 \asymp \sqrt{\lambda_1} \asymp \sigma$ for some $\sigma \coloneqq \sigma(d_1,d_2,r)$. When we take $\sigma = 1/\sqrt{d_1d_2}$ as in~\cite{lu2021low}, it suffices to show the convex hull of a subset of the vectorization of $\mathcal{X}$ contains a ball or sphere in $\R^{d_1d_2}$ with some radius which does not scale with $d_1$ or $d_2$. For example, if $\vecc{\mathcal{X}}$ is the Euclidean unit ball (sphere) in $\R^{d_1d_2}$, we can prove Assumption \ref{assu_sampling} holds by merely setting $\mathcal{D}$ as the uniform distribution:
\begin{itemize}
    \item[(i)] We write $\vecc{X} = \vx \coloneqq (\vx_1 ,\dots, \vx_{d_1d_2})$. Then we can write $\vx_i = \frac{Z_i}{\sqrt{Z_1^2 + \dots+ Z_{d_1d_2}^2}} \cdot G$ where $Z_i$ follows standard normal distribution and $G$ is an random variable in [0,1] that is independent with $Z$. Since when $T_1$ becomes larger, $G$ is more likely to get close to 1. and hence we have $\E(G^2) \geq c_1$ for some absolute constant $c_1 \in \R$ for large $T_1$. By symmetry we know $\Sigma$ should be a diagonal matrix, and $\Sigma_{ii} = \E(\vx_i^2) = \E(G^2) \E(\frac{Z_i^2}{Z_1^2 + \dots+ Z_{d_1d_2}^2}) \in \frac{1}{d_1d_2} [c_1,1]$, which imples that $\lambda_{\min}(\Sigma)=\norm{\Sigma}_2 \asymp \frac{1}{d_1d_2}$.
    \item[(ii)] To show $\sigma_X^2 \lesssim \frac{1}{d_1d_2}$, we only need to show that $\norm{\sqrt{d_1d_2}\vx_i}_{\phi_2} = O(1)$ for all $i$. It suffices to show that there exists some $t \in \R^{+}$ such that $\E\left(\exp\left\{{td_1d_2}\frac{Z_i^2}{Z_1^2 + \dots+ Z_{d_1d_2}^2}\right\}\right) < +\infty$. And we have:
    \begin{align*}
        \E(\exp\{{td_1d_2}\frac{Z_i^2}{Z_1^2 + \dots+ Z_{d_1d_2}^2}\}) &= \dfrac{\Gamma(d_1d_2)}{\Gamma(0.5)\Gamma(\frac{d_1d_2-1}{2})} \int_0^1 x^{-\frac{1}{2}}(1-x)^{\frac{d_1d_2-3}{2}} e^{tnx} dx  \\
        &\leq O(\sqrt{d_1d_2}) \int_{0}^{\infty} x^{-\frac{1}{2}} e^{[(t-\frac{1}{2})n+\frac{3}{2}]x} dx \\
        &\leq O(\sqrt{d_1d_2}) \dfrac{\Gamma(0.5)}{\sqrt{(\frac{1}{2}-t)n-\frac{3}{2}}} = O(1), \quad t \in (0,\frac{1}{2}).
    \end{align*}
\end{itemize}


Without loss of generality, we can assume that $c_- \sigma^2 \leq \{\lambda_1, \lambda_2^2\} \leq c_+ \sigma^2$ for some absolute constant $c_-, c_+$ for the simplicity of following theoretical analysis. Assumption \ref{assu_sampling} implies that if $X$ is sampled from the distribution $\mathcal{D}$, then for any $\Delta \in \R^{d_1 \times d_2}$ satisfying $\norm{\Delta}_F \leq 1$, we have:
\begin{align}
    \E[\inp{X}{\Delta}^2] &= \vecc{\Delta}^\top \Sigma \vecc{\Delta} \geq \lambda_1 \geq {c_- \, \sigma^2} \coloneqq \alpha; \label{alpha} \\
    &\E[\inp{X}{\Delta}^4] \leq 16 \lambda_2^4 \leq {16c_+^2 \, \sigma^4} \coloneqq \beta. \label{beta}
\end{align}
\item For Assumption \ref{assu_link}, we can just take the absolute constant $c_2$ as $c_2 = 2c_+/\sqrt{c_-}$ defined in Eqn. \eqref{alpha} and \eqref{beta}. And the condition $c_\mu \geq \inf_{\{|x| < {(S+2)\sigma c_2}\}} \mu^{\prime} (x) > 0$ could be easily verified since the scale of $\sigma$ is mostly small in reality.
\item Assumption \ref{assu_link} implies that $\eta_t$ given $\mathcal{F}_t$ would satisfy the sub-Gaussian condition with parameter $\sigma_\eta = \sqrt{k_\mu}$ based on Lemma \ref{lemma_glmsubg} in Appendix \ref{lemmas_glm}.
\end{enumerate}


==> app_thmlow.tex <==
\section{Theorem \ref{thm_regalg1} and its analysis}
\subsection{Theorem \ref{thm_regalg1}}
\begin{theorem} \label{thm_regalg1} \textup{(Regret of LowGLM-UCB)}
Under Assumption \ref{assu_bound} and \ref{assu_link}, for any fixed failure rate $\delta \in (0,1)$, if we run the LowGLM-UCB algorithm with $\rho_t(\delta) = \alpha_{t+T_1}(\delta/2)$ and
\begin{align}
    \lambda_\perp \asymp \dfrac{c_\mu S_0^2 T}{k \log(1+\frac{c_\mu S_0^2 T}{k \lambda_0})},  \nonumber
\end{align}
then the bound of regret for LowGLM-UCB $(Regret_{T_2})$ achieves ${\widetilde{O}(k \sqrt{T}+ T S_\perp)}$, with probability at least $1-\delta$.

\end{theorem}


\subsection{Proposition \ref{prop_mubound} with its proof}
We firstly present the following important Proposition \ref{prop_mubound} for obtaining the upper confidence bound.
\begin{proposition} \label{prop_mubound}
For any $\delta, t$ such that $\delta \in (0,1)$, $t \geq 2$, and for $\beta_t^x (\delta)$ defined in Eqn. \eqref{beta_def} and \eqref{alpha_def}, with probablity $1-\delta$, it holds that
\begin{align}
    \vert \mu(x^\top \theta^*) - \mu(x^\top \hat\theta_t)\vert \leq \beta_{t+T_1}^x(\delta), \label{prop_mubound_equ}
\end{align}
simultaneously for all $x \in \R$ and all $t \geq 2$.
\end{proposition}
\subsubsection{Technical Lemmas}
\begin{lemma} \label{lemma_goodprob} \textup{(Abbasi-Yadkori et al., 2011, Theorem 1)}
Let $\{\mathcal{F}_t\}_{t=0}^\infty$ be a filtration and $\{x_t\}_{t=0}^\infty$ be an $\mathbb{R}^d$-valued stochastic process adapted to $\mathcal{F}_t$. Let $\{\eta_t\}_{t=0}^\infty$ be a real-valued stochastic process such that $\eta_t$ is adapted to $\mathcal{F}_t$ and is conditionally $\sigma_0$-sub-Gaussian for some $\sigma_0 > 0$, i.e.
\begin{align}
    \E[\exp(\lambda \eta_t) \vert \mathcal{F}_t] \leq \exp\left( \dfrac{\lambda^2 \sigma_0^2}{2} \right), \quad \quad \forall \lambda \in \R. \nonumber
\end{align}
Consider the martingale $S_t = \sum_{k=1}^{t-1} \eta_{k} x_k$ and the process $V_t = \sum_{k=1}^{t-1} x_{k} x_{k}^{\top} + \Lambda$ when $t \geq 2$. For any $\delta > 0$, with probability at least $1-\delta$, we have the following result simultaneously for all $t \geq 2$:
\begin{align}
    \norm{S_t}_{V_t^{-1}} \leq \sigma_0 \sqrt{\log (\det(V_t)) - \log(\delta^2 \det(\Lambda))}. \nonumber
\end{align}
\end{lemma}
We omit the proof for this lemma since a lot of technical details are involved.

\begin{lemma} \label{lemma_inversepd} 
For any two symmetric positive definite matrix $A,B \in R^{p \times p}$ such that $A \preceq B$, we have $A B^{-1} A \preceq A$.
\end{lemma}
\proof Since $A \preceq B$ and both of them are invertible matrices, we have $B^{-1} \preceq A^{-1}$ directly based on positive definiteness property. Conjugate with $A$ on both sides we can directly obtain $A B^{-1} A \preceq A$. \hfill \qedsymbol

\begin{lemma} \label{lemma_valko} \textup{(Valko et al., 2014, Lemma 5)}
For any $T \geq 1$, let $V_{T+1} = \sum_{i=1}^{T} x_ix_i^{\top} + \Lambda \in R^{p}$ where $\Lambda = \text{diag}\{\lambda_1, \dots, \lambda_p\}$. And we assume that $\norm{x_i}_2 \leq S$. Then:
\begin{align}
    \log \dfrac{\vert V_{T+1} \vert}{\vert \Lambda \vert} \leq \max_{\{t_i\}_{i=1}^p} \sum_{i=1}^p \log \left(1 + \dfrac{S^2 t_i}{\lambda_i} \right), \nonumber
\end{align}
where the maximum is taken over all possible positive real numbers $\{t_i\}_{i=1}^p$ such that $\sum_{i=1}^p t_i = T$
\end{lemma}
\proof We aim to bound the determinant $\vert V_{T+1} \vert$ under the coordinate constrains $\norm{x_i}_2 \leq S$. Let's denote
\begin{align}
    U(x_1,\dots,x_T) = \lvert \Sigma + \sum_{t=1}^T x_t x_t^\top \rvert. \nonumber
\end{align}

Based on the property of the sum of rank-1 matrices (e.g. Valko et al., 2014, Lemma 4), we know that the maximum of $U(x_1,\dots,x_T)$ is reached when all $x_t$ are aligned with the axes:
\begin{align}
    U(x_1,\dots,x_T) = \max_{\substack{x_1, \dots, x_T; \\ x_t \in S \cdot \{e_1, \dots, e_N\}}} \lvert \Sigma + \sum_{t=1}^T x_t x_t^\top \rvert = \max_{\substack{t_1, \dots, t_N \text{positive integers}; \\ \sum_{i=1}^N t_i = T}} \lvert \text{diag}(\lambda_i + t_i)  \rvert \nonumber \\ 
    \leq \max_{\substack{t_1, \dots, t_N \text{positive integers}; \\ \sum_{i=1}^N t_i = S^2T}} \prod_{i=1}^N  (\lambda_i + S^2t_i). \nonumber 
\end{align} \hfill \qedsymbol

\subsubsection{Proof of Proposition \ref{prop_mubound}}
\proof Recall our definition of $g_t(\theta)$ and its gradient accordingly as 
\begin{align}
    g_t(\theta) &= \sum_{i=1}^{T_1} \mu({x_{s_1,i}}^\top{\theta}) x_{s_1,i} + \sum_{k=1}^{t-1} \mu(x_k^\top \theta) x_k + \Lambda \theta, \nonumber \\
    \nabla_\theta g_t(\theta) = \sum_{i=1}^{T_1} & \mu^\prime({x_{s_1,i}}^\top{\theta}) x_{s_1,i}x_{s_1,i}^\prime +\sum_{k=1}^{t-1} \mu^\prime (x_k^\top \theta) x_k x_k^\top + \Lambda \stackrel{\textup{(i)}}{\succeq}  c_\mu M_t(c_\mu), \label{gtgradientdef}
\end{align}
where the relation (i) holds if $\theta \in \mathit{\Theta}_0$. Based on Assumptions, we know the gradient $\nabla_\theta g_t(\theta)$ is continuous. Then the Fundamental Theorem of Calculus will imply that 
\begin{align}
    g_t(\theta^*) - g_t(\hat \theta_t) = G_t (\theta^* - \hat \theta_t), \nonumber
\end{align}
where
\begin{align}
    G_t = \int_0^1 \nabla_\theta g_t(s\theta^* + (1-s)\hat \theta_t) \, ds. \nonumber
\end{align}

Since we assume that the inverse link function $\mu(\cdot)$ is $k_\mu-$Lipshitz, and the matrix $G_t$ is always invertible due to the fact that at least we have $G_t \succeq \Lambda$, we can obtain the following result. Notice the inequality (i) comes from the fact that $G_t \succeq c_\mu M_t(c_\mu)$ and hence $M_t(c_\mu)^{-1}/c_\mu \succeq G_t^{-1}$.
\begin{align}
    \vert \mu(x^\top \theta^*) - \mu(x^\top \hat \theta_t) \vert &\leq k_\mu \vert x^\top (\theta^*-\hat \theta_t) \vert 
    = k_\mu \vert x^\top G_t^{-1} (g_t(\theta^*)-g_t(\hat \theta_t)) \vert \nonumber \\ 
    &\hspace{-12 mm}\leq k_\mu \norm{x}_{G_t^{-1}} \, \norm{g_t(\theta^*)-g_t(\hat \theta_t)}_{G_t^{-1}} \stackrel{\textup{(i)}}{\leq} 
    \frac{k_\mu}{c_\mu} \norm{x}_{M_t(c_\mu)^{-1}} \, \norm{g_t(\theta^*)-g_t(\hat \theta_t)}_{M_t(c_\mu)^{-1}}. \nonumber
\end{align}

% Next,
% \begin{align}
%     \norm{g_t(\theta^*)-g_t(\btheta_t)}_{M_t(c_\mu)^{-1}} &\leq \norm{g_t(\theta^*)-g_t(\hat \theta_t)}_{M_t(c_\mu)^{-1}} +\norm{g_t(\hat \theta_t)-g_t(\btheta_t)}_{M_t(c_\mu)^{-1}} \label{eq_interpolate} \\
%     &\leq 2 \norm{g_t(\hat \theta_t) - g_t(\theta^*)}_{M_t(c_\mu)^{-1}}, \nonumber
% \end{align}
% where the first inequality comes from the triangle inequality of the norm and the second inequality is by the definition of $\hat \theta_t$.
In addition, based on the definition of $\hat \theta_t$ in Equation \eqref{hattheta}, we have $g_t(\hat \theta_t) - g_t(\theta^*) = \sum_{k=1}^{T_1} (y_{s_1,k} - \mu(x_{s_1,k}^\top \theta^*))x_{s_1,k} + \sum_{k=1}^{t-1} (y_k - \mu(x_k^\top \theta^*))x_k - \Lambda \theta^* =\sum_{k=1}^{T_1} \eta_{s_1,k}x_{s_1,k}+ \sum_{k=1}^{t-1} \eta_kx_k - \Lambda \theta^*$. Therefore, 
\begin{align}
    \vert \mu(x^\top \theta^*) - \mu(x^\top \hat \theta_t) \vert &\leq  \frac{k_\mu}{c_\mu} \norm{x}_{M_t(c_\mu)^{-1}} \, \norm{g_t(\hat \theta_t) - g_t(\theta^*)}_{M_t^{-1}(c_\mu)} \nonumber  \\
    &\hspace{-18 mm}\leq \frac{k_\mu}{c_\mu} \norm{x}_{M_t(c_\mu)^{-1}} \, \left(\norm{\sum_{k=1}^{T_1} \eta_{s_1,k}x_{s_1,k}+\sum_{k=1}^{t-1} \eta_k x_k}_{M_t^{-1}(c_\mu)} + \norm{\Lambda \theta^*}_{M_t^{-1}(c_\mu)}\right). \label{prop_pf_1}
\end{align}

Now, let's use Lemma \ref{lemma_goodprob} to bound the term $\norm{\sum_{k=1}^{T_1} \eta_{s_1,k}x_{s_1,k}+\sum_{k=1}^{t-1} \eta_k x_k}_{M_t^{-1}(c_\mu)}$. If we define the filtration $\mathcal{F}_t \coloneqq \{\{x_t,x_{t-1},\eta_{t-1},\dots,x_1,\eta_1\} \cup \{x_{s_1,k},\eta_{s_1,k}\}_{k=1}^{T_1}\}$, then for any $\delta \in (0,1)$, with probability $1-\delta$, it holds that for all $t \geq 2$,
\begin{align}
    \norm{\sum_{k=1}^{T_1} \eta_{s_1,k}x_{s_1,k}+\sum_{k=1}^{t-1} \eta_k x_k}_{M_t^{-1}(c_\mu)} \leq \sigma_0 \sqrt{\log \left( \dfrac{\vert M_t(c_\mu)\vert}{\vert  \frac{\Lambda}{c_\mu} \vert } \right) - 2 \log (\delta)}, \nonumber
\end{align}
where based on Lemma \ref{lemma_valko},
\begin{align}
  \log \left( \dfrac{\vert M_t(c_\mu)\vert}{\vert  \frac{\Lambda}{c_\mu} \vert } \right) & \leq \max_{\substack{t_i \geq 0, \\  \sum_{i=1}^t t_i = t+T_1}} \sum_{i=1}^p \log \left(1 + \dfrac{c_\mu S_0^2 t_i}{\lambda_i} \right) \nonumber \\ 
&\leq k \log \left(1+\frac{c_\mu S_0^2}{k \lambda_0}(t+T_1) \right) + (d-k) \log \left( 1 + \frac{c_\mu S_0^2}{(d-k) \lambda_\perp}(t+T_1)\right)\nonumber \\ &\leq  k \log \left(1+\frac{c_\mu S_0^2}{k \lambda_0}(t+T_1) \right) +  \frac{c_\mu S_0^2}{\lambda_\perp}(t+T_1). \label{prop_pf_2}
\end{align}

And next by Lemma \ref{lemma_inversepd}, we have
\begin{align}
    \norm{\Lambda \theta^*}_{M_t^{-1}(c_\mu)} = c_\mu \norm{\frac{\Lambda}{c_\mu} \, \theta^*}_{M_t^{-1}(c_\mu)} \leq \sqrt{c_\mu} \norm{\theta^*}_{\Lambda} \leq \sqrt{c_\mu}(\sqrt{\lambda_0}S_0 + \sqrt{\lambda_\perp} S_\perp). \label{prop_pf_3}
\end{align}

Combine Equation \eqref{prop_pf_2} and \eqref{prop_pf_3} into Equation \eqref{prop_pf_1}, we finish our proof. \hfill \qedsymbol
\par Since Equation \eqref{prop_mubound_equ} in Proposition \ref{prop_mubound} holds simultaneously for all $x \in \R$ and $t \geq 1$, the following conclusion holds.
\begin{corollary} \label{coro_rvbound}
For any random variable $z$ defined in $\R$, we have the following holds
\begin{align}
     \vert \mu(z^\top \theta^*) - \mu(z^\top \hat\theta_t)\vert \leq \beta_{t+T_1}^z(\delta), \nonumber
\end{align}
with probability at least $1-\delta$. Furthermore, for any sequence of random variable $\{z_t\}_{t=2}^{T}$, with probability $1-\delta$ it holds that
\begin{align}
     \vert \mu(z_t^\top \theta^*) - \mu(z_t^\top \hat\theta_t)\vert \leq \beta_{t+T_1}^{z_t}(\delta), \nonumber
\end{align}
simultaneously for all $t \geq 1$.
\end{corollary}
\subsection{Proposition \ref{prop_mubound2} with its proof}
We denote the optimal action $x^* = \arg \max_{x \in \mathcal{X}_0} \mu(x^\top \theta^*)$. 
\begin{proposition} \label{prop_mubound2}
For all $\delta \in (0,1)$, with probability $1 - \delta$, it holds that
\begin{align}
    \mu({x^*}^\top \theta^*) - \mu(x_t^\top \theta^*) \leq 2 \beta_{t+T_1}^{x_t}\left(\frac{\delta}{2}\right), \nonumber
\end{align}
simultaneously for all $t \in \{2,3,\dots,T_2\}$.
\end{proposition}
\proof According to Corollary \ref{coro_rvbound}, outside of the event of measure can be bounded by $\delta/2$:
\begin{align}
    \mu(x_t^\top \hat\theta_t) - \mu(x_t^\top \theta^*) \leq \beta_{t+T_1}^{x_t}\left(\frac{\delta}{2}\right) \quad \text{for all } t \in \{2,3,\dots,T_2\}. \nonumber
\end{align}
Similarly, with probability at least $1-\delta/2$ it holds that
\begin{align}
    \mu(x^*{}^\top \theta^*) - \mu(x^*{}^\top \hat\theta_t) \leq \beta_{t+T_1}^{x^*}\left(\frac{\delta}{2}\right) \quad \text{for all } t \in \{2,3,\dots,T_2\}. \nonumber
\end{align}
Besides, by the choice of $x_t$ in Algorithm \ref{alg1}
\begin{align}
    \mu(x^*{}^\top \hat\theta_t) - \mu(x_t^\top \hat\theta_t) &= \mu(x^*{}^\top \hat\theta_t) + \beta_{t+T_1}^{x^*}\left(\frac{\delta}{2}\right) - \mu(x_t^\top \hat\theta_t) - \beta_{t+T_1}^{x^*}\left(\frac{\delta}{2}\right) \nonumber \\ 
    & \leq  \mu(x_t^\top \hat\theta_t) + \beta_{t+T_1}^{x_t}\left(\frac{\delta}{2}\right) - \mu(x_t^\top \hat\theta_t) - \beta_{t+T_1}^{x^*}\left(\frac{\delta}{2}\right) \nonumber \\ &= \beta_{t+T_1}^{x_t}\left(\frac{\delta}{2}\right) - \beta_{t+T_1}^{x^*}\left(\frac{\delta}{2}\right). \nonumber
\end{align}

By combining the former inequalities we finish our proof. \hfill \qedsymbol

\subsection{Proof of Theorem \ref{thm_regalg1}}
\proof Based on Proposition \ref{prop_mubound2} we have
\begin{align}
    \mu({x^*}^\top \theta^*) - \mu(x_t^\top \theta^*) \leq 2 \beta_{{t+T_1}}^{x_t}\left(\frac{\delta}{2}\right)
 = 2 \alpha_{{t+T_1}}\left(\frac{\delta}{2}\right)
 \norm{x_t}_{M_t^{-1}(c_\mu)} \leq 2 \alpha_{T}\left(\frac{\delta}{2}\right)
 \norm{x_t}_{M_t^{-1}(c_\mu)}. \nonumber
\end{align}

Since we know that $\mu({x^*}^\top \theta^*) - \mu(x^\top \theta^*) \leq k_\mu({x^*}^\top \theta^* - x^\top \theta^*) \leq 2 k_\mu S_0^2$ for all possible action $x$, and we can safely expect that $\alpha_{T_2}(\delta/2) > k_\mu S_0^2$ (at least by choosing $\sigma_0 = k_\mu \max\{S_0^2,1\}$), then the regret of Algorithm \ref{alg1} can be bounded as
\begin{align}
    Regret_{T_2} &\leq 2 k_\mu S_0^2 + \sum_{t=2}^{T_2} \min\{\mu({x^*}^\top \theta^*) - \mu(x_t^\top \theta^*), 2 k_\mu S_0^2\} \nonumber \\ 
    &\leq 2 k_\mu S_0^2 + 2 \alpha_{T}\left(\frac{\delta}{2}\right) \sum_{t=2}^{T_2} \min\{\norm{x_t}_{M_t^{-1}(c_\mu)}, 1\} \nonumber \\ 
    &\stackrel{\textup{(i)}}{\leq} 2 k_\mu S_0^2 + 2 \alpha_{T}\left(\frac{\delta}{2}\right)\sqrt{T_2} \sqrt{\sum_{t=2}^{T_2} \min\{\norm{x_t}_{M_t^{-1}(c_\mu)}^2, 1\}}. \nonumber
\end{align}
where the ineuqlity (i) comes from Cauchy-Schwarz inequality. And a commonly-used fact (e.g.~\cite{abbasi2011improved}, Lemma 11) yields that
\begin{align}
    \sum_{i=2}^{t}\min\{\norm{x_i}_{M_i^{-1}(c_\mu)}^2, 1\} &\leq 2 \log\left( \dfrac{\vert M_{t+1}(c_\mu)\vert}{\vert M_{2}(c_\mu) \vert} \right) \leq  2\log\left( \dfrac{\vert M_{t+1}(c_\mu)\vert}{\vert \frac{\Lambda}{c_\mu} \vert} \right) \nonumber \\
    &\leq  k \log \left(1+\frac{c_\mu S_0^2}{k \lambda_0}(t+T_1) \right) +  \frac{c_\mu S_0^2}{\lambda_\perp}(t+T_1). \nonumber
\end{align}

Finally, by using the argument in Eqn. \eqref{prop_pf_2} and then plugging in the chosen value for $\lambda_\perp = \dfrac{c_\mu S_0^2 T}{k \log(1+\frac{c_\mu S_0^2 T}{k \lambda_0})}$, we have  
\begin{align}
    &Regret_{T_2} \leq 2 k_\mu S_0^2 + \nonumber \\ 
    &\frac{2k_\mu}{c_\mu} \left(\sigma_0 \sqrt{2k \log \left(1 + \frac{c_\mu S_0^2}{k \lambda_0}T \right) - 2\log \left(\frac{\delta}{2}\right)} +  \sqrt{c_\mu}\left(\sqrt{\lambda_0} S_0 + \sqrt{\frac{c_\mu S_0^2 T}{k\log \left(1 + \frac{c_\mu S_0^2}{k \lambda_0}T \right)}}S_\perp\right)\right) \nonumber \\
    &\times \sqrt{T_2} \sqrt{4k\log \left(1 + \frac{c_\mu S_0^2}{k \lambda_0}T \right)}, \nonumber
\end{align}
which gives us the final bound in Theorem \ref{thm_regalg1}. \hfill \qedsymbol





==> checklist.tex <==

\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss the limitation of our first algorithm G-ESTT in the beginning of Subsection \ref{subsec:gestt}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}



==> plowglmucb.tex <==
A potential issue of Algorithm \ref{alg1} is that in each iteration we need to calculate the parameter estimate $\btheta_t$ involving a projection procedure, which could be computationally expensive. Inspired by some related discussion in~\cite{abbasi2011improved}, we could only recompute $\hat\theta_t$ and $\btheta_t$ whenever $\vert M_t(c_\mu)\vert$ increases by a constant factor $C > 1$ in scale, and consequently we only need to solve the Eqn. \eqref{hattheta} for only $O(\log(T_2))$ times up to the horizon $T_2$, which remarkably helps save the computation. And at the same time, the theoretical bound of the regret only increase up to a multiplier $\sqrt{C}$, which is essentially in the same scale. We call this modified version LowGLM-UCB method as Parsimonious LowGLM-UCB (PLowGLM-UCB). Its pseudo-code is given in Algorithm \ref{alg2}.

\begin{algorithm}
\caption{PLowGLM-UCB} \label{alg2}
\begin{algorithmic}[1] 
\Input $T_2,k,\mathcal{X}_0$, the probability rate $\delta$, penalization parameters $(\lambda_0,\lambda_\perp)$, the constant $C$.
\State Play an arm $x_1$ arbitrarily and receive the reward $y_1$. Initialize $M_2(c_\mu) = x_1 x_1^\top + \Lambda/c_\mu$
\For{$t \geq 2$}
\If{$\vert M_t(c_\mu)\vert > C \vert M_\tau (c_\mu)\vert$}
\State Estimate $\hat \theta_t$ according to \eqref{hattheta}.
\IfThenElse{$\hat \theta_t \in \mathit{\Theta}_0$}{$\btheta_t = \hat \theta_t$}{compute $\btheta_t$ according to \eqref{ttheta}}.
\State $\tau = t$
\EndIf
\State Choose arm $x_t = \arg\max_{x \in \mathcal{X}_0} \{\mu({x}^\top{\btheta_\tau}) + \rho_{\tau}(\delta)\norm{x}_{M_t^{-1}(c_\mu)} \}$, receive $y_t$.
\State Update $M_{t+1}(c_\mu) \longleftarrow M_{t}(c_\mu) + x_t x_t^\top$.
\EndFor
\end{algorithmic}
\end{algorithm}
\noindent \textbf{Regret bound.} Theorem \ref{thm_regalg2} shows the regret bound of PLowGLM-UCB under Assumption \ref{assu_bound} and \ref{assu_link}.
\begin{theorem} \label{thm_regalg2} \textup{(Regret of PLowGLM-UCB)}
For any fixed failure rate $\delta \in (0,1)$, if we run the PLowGLM-UCB algorithm with $\rho_t(\delta) = \alpha_t(\delta/2)$ and
\begin{align}
    \lambda_\perp = \dfrac{c_\mu S^2 T_2}{k \log(1+\frac{c_\mu S^2 T_2}{k \lambda_0})} \; \;  (\textup{or }\lambda_\perp \asymp \dfrac{c_\mu S^2 T_2}{k \log(1+\frac{c_\mu S^2 T_2}{k \lambda_0})} ). \nonumber
\end{align}
Then the regret of PLowGLM-UCB $(Regret_{T_2})$ satisfies, with probability at least $1-\delta$
\begin{align}
    \tilde{O}(k \sqrt{T_2} + \sqrt{ \lambda_0 k T_2} \, + T_2 S_\perp) \sqrt{C} {\color{red} = \tilde{O}(k \sqrt{T_2}+ T_2 S_\perp)}. \nonumber
\end{align}
\end{theorem}
Similarly, we can get the bound of regret for PLowGLM-UCB in problem dependence case, and the bound will be exactly the same as that we have shown in Theorem \ref{thm_pdregalg1} except a constant multiplier $\sqrt{C}$.
\begin{remark} \label{rem_cmu}
Technically we can always assume $c_\mu \in (0,1]$ since we can always choose $c_\mu = 1$ when it can take values greater than $1$. And hence here for both LowGLM-UCB and PLowGLM-UCB, we can just use $V_t$ instead of $M_t(c_\mu)$ for the projection step in Eqn. \eqref{ttheta}. And the bound of the regret would only increase by a constant factor of $1/\sqrt{c_\mu}$. Detailed explanation is deferred to Appendix \ref{sec:app:remark}.
\end{remark}
